Graphlets as Building Blocks for Structural Vocabulary in Knowledge Graph Foundation Models

Foundation models excel at language, where sentences become tokens, and vision, where images become pixels, because both reduce to discrete symbols on a shared, fixed grid. Knowledge Graphs share the discreteness, but not the geometry. Their entities and relations are discrete symbols, yet their arrangement is relational and lacks a common, fixed grid. Knowledge Graphs (KGs) share the discreteness, but not the geometry. They form irregular, non-Euclidean topologies whose local neighborhoods differ from graph to graph. Therefore, Knowledge Graph Foundation Models (KGFMs) rely on identifying structural invariances to produce transferable representations. Without a universal token set, KGFMs are limited in their ability to transfer representations across unseen KGs. We close this gap by treating graphlets, small connected graphs, as structural tokens that recur in heterogeneous KGs. In this paper, We introduce a model-agnostic framework based on a vocabulary of graphlets that mines a KG between relations via pattern matching. In particular, we considered closed and open 2- and 3-path, and star graphlets, to obtain robust invariances. The framework is evaluated on 51 KGs from a wide range of domains, for zero-shot inductive and transductive link prediction. Experiments show that adding simple graphlets to the vocabulary yields models that outperform prior KGFMs.

==> extension_of_the_structural_vocabulary_definition.tex <==
\section{Extension of the Structural Vocabulary Definition}
The presented methodology can be extended to a more general structural vocabulary. As we use pattern matching with SPARQL the vocabulary can consist of any pattern expressible by SPARQL.

A slight extension of definition \ref{def:graphlet} includes the definition of a set of negative triples that cannot be contained in a neighborhood of an occurence.

\begin{definition}\label{def:graphlet-neg}
A graphlet $\cG$ is a tuple $(G, \cT_-)$ consisting of a connected Knowledge graph $G=(\cE, \cR, \cT)$ and a set of negative triples $\cT_-$ with $G\setminus \cT _ -$ is connected. A graphlet $\cG$ occurs in a KG $K=(\cE^K,\cR^K,\cT^K_+)$ if and only if there is a subgraph $K'=(\cE', \cR', \cT'_+)\subset K$ that is isomorphic to $G_+=(\cE, \cR, \cT\setminus \cT_-)$, if additionally $\cT_-\neq \emptyset$ there must not be a subgraph $\hat{K}\subset K$ that contains $K'$ that is isomorphic to $G$. $K'$ is called an occurrence of $\cG$ in $K$ and the set of occurrences is denoted by $\Phi_{\cG}(K).$
The order of a graphlet $G$ is the number of its edges $ord(G) = \norm{\cT}$.
\end{definition}
